Algorithmic amplification of biases on Google Search

The evolution of information-seeking processes, driven by search engines like Google, has transformed the access to information people have. This paper investigates how individuals' preexisting attitudes influence the modern information-seeking process, specifically the results presented by Google Search. Through a comprehensive study involving surveys and information-seeking tasks focusing on the topic of abortion, the paper provides four crucial insights: 1) Individuals with opposing attitudes on abortion receive different search results. 2) Individuals express their beliefs in their choice of vocabulary used in formulating the search queries, shaping the outcome of the search. 3) Additionally, the user's search history contributes to divergent results among those with opposing attitudes. 4) Google Search engine reinforces preexisting beliefs in search results. Overall, this study provides insights into the interplay between human biases and algorithmic processes, highlighting the potential for information polarization in modern information-seeking processes.

==> texfiles/methods.tex <==
\section{Methods}
\label{sec:methods}
\subsection{Permutation tests}

The permutation test compares the difference between the two distributions with
the differences between random permutations of the distributions together. This
process generates a distribution of test statistics under the null hypothesis of
no group difference. The p-value is determined by the proportion of permuted
test statistics that are greater than the observed statistic, thereby providing
an exact significance level without making strong parametric assumptions about
the underlying data distribution. We use the permutation test to determine
differences between characteristics of queries or results between the two groups
of participants, formed based on surveyed variables. We determine a
statistically different distribution of characteristics between the two groups
(in many cases pro-life and pro-choice) by comparing their differences with the
differences obtained from 10,000 randomly permuted groups. If the difference
measured between our two groups is larger than those observed in 9,500 of the
random permutations, we claim that the two groups have statistically significant
differences (since p < .05).

\subsection{Linear regressions}
We use a linear regression model to understand whether the extracted signals
from queries can explain a user’s abortion stance. This approach uses the
extracted implicit signals (semantics, vocabulary, and writing styles) contained
in queries as the independent variable in a linear regression model to predict
the user’s abortion stance. A high R2 value and significant f-values suggest
that the implicit signal can predict the user’s stance. We also use the
regression model coefficients to uncover how, and which extracted implicit
signals are associated with abortion stances.

\subsection{Mediation Analysis}
In this section, we describe how we use mediation analysis to determine the
relationship between the abortion attitudes towards the search queries they
write and the search results they receive. More specifically, we measure the
influence of participants’ abortion attitudes 1) directly on the search results
participants receive and 2) indirectly on the search results through its
influence on how participants write search queries. Before we measure this
relationship, we first convert the search queries and search results into
numerical values that are representative and can be used to measure the
influence of abortion attitudes.

We seek to measure whether abortion attitudes influence the search results users
receive and whether this influence is indirect through how they write queries. A
proxy to measure this difference is to first measure how different the results
are from a baseline. We consider search results presented to participants with
neutral attitudes toward abortion as the baseline. Deviation from this baseline
represents the search results. Our analysis essentially measures how abortion
attitudes influence the deviation of search results from the search results
shown to participants with neutral attitudes toward abortion. Similarly, we
represent search queries in our model with their deviation from search queries
written by participants with neutral attitudes toward abortion. Given the
multiple components of search results (titles, snippets, and domains) and search
queries (vocabulary, style, domains), we aim to investigate the influence of
each representation separately.

